HarmonySet: A Comprehensive Dataset for Understanding Video-Music Semantic Alignment and Temporal Synchronization

This paper introduces HarmonySet, a comprehensive dataset designed to advance video-music understanding. HarmonySet consists of 48,328 diverse video-music pairs, annotated with detailed information on rhythmic synchronization, emotional alignment, thematic coherence, and cultural relevance. We propose a multi-step human-machine collaborative framework for efficient annotation, combining human insights with machine-generated descriptions to identify key transitions and assess alignment across multiple dimensions. Additionally, we introduce a novel evaluation framework with tasks and metrics to assess the multi-dimensional alignment of video and music, including rhythm, emotion, theme, and cultural context. Our extensive experiments demonstrate that HarmonySet, along with the proposed evaluation framework, significantly improves the ability of multimodal models to capture and analyze the intricate relationships between video and music.

==> table/ablation_egogpt.tex <==
\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1.0}
    \caption{\textbf{Ablation Study on EgoGPT.} We construct different EgoRAG memory banks using generated captions from EgoGPT variants. The first three rows use captions from human annotations as a reference. All response generation models utilize EgoGPT (EgoIT-99K+D1) to ensure fair comparison. The result indicates how caption quality affects of EgoBulter performance.}
    \scriptsize
    \vspace{-8pt}
    \resizebox{\linewidth}{!}{%
     \begin{tabular}{lcclc}
\toprule
% \multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{Visual Input}} & \multirow{2}{*}{\textbf{Audio Input}} & \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{6}{c}{\textbf{EgoLifeQA}} \\ 
Caption Source & \textbf{Visual} & \textbf{Audio} & \textbf{Dataset} & \textbf{Avg.} \\ \midrule
Narration               & \textcolor{teal}{\checkmark}  &  \textcolor{teal}{\checkmark}   & - &    31.5       \\
Transcript              & \textcolor{red}{\ding{55}}  &  \textcolor{teal}{\checkmark}  &   -&    29.6       \\
Visual-Audio Caption  &\textcolor{teal}{\checkmark}  & \textcolor{teal}{\checkmark} & - &    45.5       \\ \midrule
EgoGPT (Audio Only)     &  \textcolor{red}{\ding{55}} & \textcolor{teal}{\checkmark} & EgoIT-99K  &    27.2       \\
EgoGPT (Audio Only)     &  \textcolor{red}{\ding{55}} & \textcolor{teal}{\checkmark} & EgoIT-99K+D1  &   28.1      \\
EgoGPT (Visual Only)    &  \textcolor{teal}{\checkmark}  &  \textcolor{red}{\ding{55}} & EgoIT-99K  &    31.2     \\
EgoGPT (Visual Only)    &  \textcolor{teal}{\checkmark}  &  \textcolor{red}{\ding{55}} & EgoIT-99K+D1  &  33.6   \\\midrule
EgoGPT (Visual+Audio)   &  \textcolor{teal}{\checkmark} &  \textcolor{teal}{\checkmark}  & EgoIT-99K  &   33.1    \\
EgoGPT (Visual+Audio)   & \textcolor{teal}{\checkmark}   &  \textcolor{teal}{\checkmark}   & EgoIT-99K+D1  &   36.0    \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\label{tab:ablation_gpt}
\end{table}


==> table/ablation_egorag.tex <==
\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1.0}
    \caption{\textbf{Effectiveness of EgoRAG.} Integrating EgoRAG significantly enhances video-language models' performance in long-context question answering, especially for questions requiring longer certification lengths. For comparison, we evaluate Gemini-1.5-Pro and EgoGPT on a half-hour video segment, limiting their answers to this timeframe.}
    \scriptsize
    \vspace{-8pt}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{Certificate Length}} \\ 
&  \textbf{$<2h$} & \textbf{$2h-6h$} & \textbf{$6h-24h$} & \textbf{$>24h$}  \\ 
\midrule
Gemini-1.5-Pro    & 27.9         & 14.8            & 25.0             & 18.4   \\
EgoGPT            & 28.2         & 29.1            & 26.8             & 25.0     \\
\midrule
EgoGPT+EgoRAG   & 27.2         & 35.7            & 38.9             & 35.4  \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\label{tab:ablation_rag}
\end{table}

==> table/egoit.tex <==
\begin{table}[t]
\centering
% \vspace{-10pt}
\caption{\textbf{Dataset Composition of EgoIT-99K.} We curated 9 classic egocentric video datasets and leveraged their annotations to generate captioning and QA instruction-tuning data for fine-tuning EgoGPT, building on the LLaVA-OneVision base model~\cite{li2024llava}. \textbf{\#AV} means the number of videos with audio used for training. QAs include multiple types -
\textbf{VC}: Video Captioning, \textbf{AVC}: Audio-Video Captioning, \textbf{MCQ}: Multiple Choice Questions, \textbf{MRC}: Multi-Round Questions, \textbf{IQA}: Image Question-Answering.}
\label{tab:egoit}
\vspace{-5pt}
\setlength\tabcolsep{8pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccl}
\toprule
\textbf{Dataset} & \textbf{Duration} & \textbf{\#Videos (\#AV)} & \textbf{\#QA} & \textbf{QA Type} \\ 
\midrule
Ego4D~\cite{ego4d}       & 3.34h & 523 (458) & 1.41K & VC, AVC, MCQ, MRC \\ 
Charades-Ego~\cite{chardesego}    & 5.04h & 591 (228) & 18.46K & VC, AVC, MRC \\ 
HoloAssist~\cite{wang2023holoassist}      & 9.17h & 121 & 33.96K & VC, MCQ, MRC, IQA \\
EGTEA Gaze+~\cite{egtea_gaze_p}     & 3.01h & 16 & 11.20K & VC, MCQ, MRC, IQA \\ 
IndustReal~\cite{schoonbeek2024industreal}      & 2.96h & 44 & 11.58K & VC, MCQ, MRC, IQA \\ 
EgoTaskQA~\cite{jia2022egotaskqa}       & 8.72h & 172 & 3.59K & VC, MCQ, MRC \\ 
EgoProceL~\cite{EgoProceLECCV2022}       & 3.11h & 18 & 5.90K & VC, MCQ, MRC, IQA \\ 
Epic-Kitchens~\cite{epickitchen}    & 4.15h & 36 & 10.15K & VC, MCQ, MRC, IQA \\ 
ADL~\cite{ADL}             & 3.66h & 8 & 3.23K & VC, MCQ, MRC, IQA \\ 
\midrule
\textbf{Total}  & \textbf{43.16h} &\textbf{1529 (686)} &\textbf{99.48K} & \\ 
\bottomrule
\end{tabular}%
}
\vspace{-15pt}
\end{table}

==> table/exp_egoit.tex <==
\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{2pt}
    \vspace{-10pt}
    \renewcommand{\arraystretch}{1.0}
    \caption{\textbf{Performance of EgoGPT.} The table compares EgoGPT with state-of-the-art commercial and open-source models on existing egocentric benchmarks.}
    \scriptsize
    \vspace{-8pt}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcc|ccc}
\toprule
{\textbf{Model}} & {\textbf{\#Param}}  & {\textbf{\#Frames}}  & {\textbf{EgoSchema}} & {\textbf{EgoPlan}} & {\textbf{EgoThink}}  \\  
\midrule
GPT-4v~\cite{openai2023gpt4v}    &     -        &   32     &     56.6      &    38.0   &     65.5       \\ 
Gemini-1.5-Pro~\cite{geminiteam2024geminifamilyhighlycapable}   &  -   &   32         &   72.2     &         31.3           &       62.4            \\ 
GPT-4o~\cite{openai2024gpt4o}                &    -       &     32    &   72.2               &     32.8              & 65.5   \\ 
\midrule
LLaVA-Next-Video~\cite{zhang2024llavanextvideo}      &    7B       &     32     &     49.7         &      29.0               &        40.6         \\
LongVA~\cite{zhang2024longva}              &  7B  &       32     &         44.1            &      29.9           &     48.3       \\
IXC-2.5~\cite{zhang2023internlmxcomposervisionlanguagelargemodel}               &   7B     &    32     &    54.6              &        29.4            &   56.0       \\
InternVideo2~\cite{wang2024internvideo2scalingfoundationmodels}     &  8B        &      32     &     55.2    &     27.5              &     43.9      \\ 
Qwen2-VL~\cite{chu2024qwen2}         &    7B       &    32   &     66.7       &        34.3        &     59.3           \\
Oryx~\cite{liu2024oryx} & 7B &  32  & 56.0 & 33.2 & 53.1  \\
LLaVA-OV~\cite{li2024llava}              &   7B     &   32     &     60.1      &       30.7             &      54.2  \\
LLaVA-Videos~\cite{zhang2024videoinstructiontuningsynthetic}        &    7B       &   32    &     57.3             &    33.6          &       56.4         \\
\midrule
EgoGPT (EgoIT)  &  7B  &   32    &   73.2 &    32.4        &   61.7  \\
EgoGPT (EgoIT+EgoLifeD1)  &  7B  &    32    & 75.4    &  33.4        &  61.4     \\
\bottomrule
\end{tabular}
}
\vspace{-15pt}
\label{tab:egogpt}
\end{table}


==> table/exp_egolife.tex <==
\begin{table*}[t!]
    \centering
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.0}
    \caption{\textbf{Performance comparison of EgoGPT with state-of-the-art models on EgoLifeQA benchmarks.} For a fair comparison on EgoLifeQA, EgoGPT was replaced with the corresponding models in the EgoButler pipeline to evaluate their performance under the same conditions. Models that provide captions for EgoLifeQA use 1 FPS for video sampling.}
    \scriptsize
    \vspace{-8pt}
    \resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\#Frames}} & \multirow{2}{*}{\textbf{Audio}} & \multirow{2}{*}{\textbf{Identity}} & \multicolumn{6}{c}{\textbf{EgoLifeQA}} \\ 
& & & & \textbf{EntityLog} & \textbf{EventRecall} & \textbf{HabitInsight} & \textbf{RelationMap} & \textbf{TaskMaster} & \textbf{Average} \\ 
\midrule
Gemini-1.5-Pro~\cite{geminiteam2024geminifamilyhighlycapable}  &  -  &   \textcolor{teal}{\checkmark}   &   \textcolor{red}{\ding{55}}   & 36.0  & 37.3  & 45.9  & 30.4  & 34.9  & 36.9  \\ 
GPT-4o~\cite{openai2024gpt4o}   &   1 FPS   &   \textcolor{red}{\ding{55}}   &   \textcolor{red}{\ding{55}}   & 34.4  & 42.1  & 29.5  & 30.4  & 44.4  & 36.2  \\ 
LLaVA-OV~\cite{li2024llava}   &   1 FPS   &   \textcolor{red}{\ding{55}}   &   \textcolor{red}{\ding{55}}   & 36.8  & 34.9  & 31.1  & 22.4  & 28.6  & 30.8  \\
\midrule
EgoGPT (EgoIT-99K)  &  1 FPS   &   \textcolor{teal}{\checkmark}   &   \textcolor{red}{\ding{55}}   & 35.2  & 36.5  & 27.9  & 29.6  & 36.5  & 33.1  \\
EgoGPT (EgoIT-99K+D1)  &  1 FPS   &   \textcolor{teal}{\checkmark}   &   \textcolor{teal}{\checkmark}   & 39.2  & 36.5  & 31.1  & 33.6  & 39.7  & 36.0  \\
\bottomrule
\end{tabular}

}
\vspace{-10pt}
\label{tab:exp_egorag}
\end{table*}


==> table/main_exp.tex <==
\begin{table*}[t!]
    \centering
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.0}
    \caption{\textbf{Performance comparison of EgoGPT with state-of-the-art commercial and open-source models on egocentric benchmarks.} For a fair comparison on EgoLifeQA, EgoGPT was replaced with the corresponding models in the EgoButler pipeline to evaluate their performance under the same conditions. Acronyms under EgoTaskQA refer to the subtasks outlined in Section~\ref{sec:egolifeqa}, such as ``En." for EntityLog, \textit{etc.} Models that provide captions for EgoLifeQA use 1 FPS for video sampling, while samples 32 frames on other benchmarks.}
    \scriptsize
    \vspace{-8pt}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lcccc|ccc|ccccccc}
\toprule
\multirow{2}{*}{\textbf{}} & \multirow{2}{*}{\textbf{\#Param}} & \multirow{2}{*}{\textbf{Release Date}}  & \multirow{2}{*}{\textbf{\#Frames}} & \multirow{2}{*}{\textbf{Audio}} & \multirow{2}{*}{\textbf{EgoSchema}} & \multirow{2}{*}{\textbf{EgoPlan}} & \multirow{2}{*}{\textbf{EgoThink}} & \multicolumn{6}{c}{\textbf{EgoLifeQA}} \\ 
\textbf{}            &        &            &           &         &                   &                   &                   & \textbf{En.} & \textbf{Ev.} & \textbf{Ha.} & \textbf{Re.} & \textbf{Ta.} & \textbf{Avg.} \\ \midrule
GPT-4v~\cite{openai2023gpt4v}    &     -       &     2023.09     &   32 / 1FPS   &   \textcolor{red}{\ding{55}}     &     56.6      &    38.0   &     65.5               & 45.8                   & 34.1                      & 41.7                       & 20.6                      & 39.1                     & 37.9                    \\ 
Gemini-1.5-Pro~\cite{geminiteam2024geminifamilyhighlycapable}   &  -  &  2024.02  &   32 / -        &   \textcolor{teal}{\checkmark}   &   72.2     &         31.3           &       62.4            & 47.3                   & 51.7                      & 42.1                       & 22.8                      & 44.2                     & 41.7          \\ 
GPT-4o~\cite{openai2024gpt4o}                &    -        &    2024.05    &     32 / 1FPS   &   \textcolor{red}{\ding{55}}        &   72.2               &     32.8              & 65.5   & 48.1                   & 41.5                      & 40.8                       & 24.9                      & 39.5                     & 39.0         \\ 
\midrule
LLaVA-Next-Video~\cite{zhang2024llavanextvideo}      &    7B       &  2024.04   &     32 / 1FPS    &   \textcolor{red}{\ding{55}}             &     49.7         &      29.0               &        40.6         & 29.4 & 25.9 & 34.1 & 23.8 & 30.3 & 28.7              \\
LongVA~\cite{zhang2024longva}              &  7B  &   2024.06    &      32 / 1FPS    &   \textcolor{red}{\ding{55}}     &         44.1            &      29.9           &     48.3       & 29.1 & 21.8 & 31.3 & 20.5 & 28.9 & 26.3           \\
IXC-2.5~\cite{zhang2023internlmxcomposervisionlanguagelargemodel}               &   7B     &   2024.07   &    32 / 1FPS    &   \textcolor{red}{\ding{55}}          &    54.6              &        29.4            &   56.0       & 35.9 & 29.2 & 36.4 & 24.3 & 33.8 & 31.9             \\
LLaVA-OV~\cite{li2024llava}              &   7B     &    2024.08  &   32 / 1FPS    &   \textcolor{red}{\ding{55}}       &     60.1      &       30.7             &      54.2  & 34.2 & 29.4 & 37.9 & 25.3 & 34.1 & 32.2        \\
InternVideo2~\cite{wang2024internvideo2scalingfoundationmodels}     &  8B        &     2024.08 &     32 / 1FPS    &   \textcolor{red}{\ding{55}}     &     55.2    &     27.5              &     43.9             & 31.8 & 27.6 & 35.0 & 21.9 & 33.1 & 29.9    \\ 
Qwen2-VL~\cite{chu2024qwen2}         &    7B       &      2024.09  &    32 / 1FPS  &   \textcolor{red}{\ding{55}}  &     66.7       &        34.3        &     59.3           & 37.6 & 30.7 & 36.2 & 24.8 & 37.9 & 33.4          \\
Oryx~\cite{liu2024oryx} & 7B & 2024.09 & 32 / 1FPS & \textcolor{red}{\ding{55}} & 56.0 & 33.2 & 53.1 & xxx & xxx & xxx & xxx & xxx &xxx \\
LLaVA-Videos~\cite{zhang2024videoinstructiontuningsynthetic}        &    7B       &    2024.09   &  32 / 1FPS   &   \textcolor{red}{\ding{55}}  &     57.3             &    33.6          &       56.4         & 36.5                   & 34.4                      & 34.9                       & 20.8                      & 34.7                     & 32.3      \\
\midrule
EgoGPT (EgoIT-99K)  &  7B  &   2024.11      &  32 / 1FPS   &   \textcolor{teal}{\checkmark} &   74.5 &    36.8        &   58.1  & 50.1                   & 49.5                      & 43.1                       & 23.5                      & 41.5                     & 41.5            \\
EgoGPT (EgoIT-99K+D1)  &  7B  &   2024.11      &    32  / 1FPS  &   \textcolor{teal}{\checkmark} & 72.8    &  36.4        &  57.5     & 52.9                   & 54.9                      & 45.1                       & 39.2                      & 48.4                     & 48.0          \\
\bottomrule
\end{tabular}
}
\vspace{-15pt}
\label{tab:model_comparison}
\end{table*}
